MedAgentGym: A Scalable Agentic Training Environment for Code-Centric Reasoning in Biomedical Data Science

We introduce MedAgentGym, a scalable and interactive training environment designed to enhance coding-based biomedical reasoning capabilities in large language model (LLM) agents. MedAgentGym comprises 72,413 task instances across 129 categories derived from 12 authentic real-world biomedical scenarios. Tasks are encapsulated within executable sandbox environments, each featuring detailed task specifications, interactive feedback mechanisms, verifiable ground truth annotations, and scalable training trajectory generation. Extensive benchmarking of 29 LLMs reveals substantial performance disparities in biomedical data science between commercial and open-source LLMs. Leveraging efficient multi-threaded and multi-turn trajectory sampling in MedAgentGym, Med-Copilot achieves performance gains of +43.02% and +45.28% from offline and online reinforcement learning, respectively, demonstrating MedAgentGym as an effective training ground while establishing itself as a cost-effective, privacy-preserving alternative competitive with proprietary LLMs (gpt-4o). By offering a unified execution environment with a comprehensive benchmark and accessible, extensible training resources, MedAgentGym delivers an integrated platform to develop LLM-based coding assistants for advanced biomedical data science.

==> table/tab-case.tex <==
\begin{table*}[!htbp]
\centering
\caption{A case study comparing an incorrect versus a correct code generation for a bioinformatics task. The incorrect code fails to account for variable ploidy in female samples, a critical edge case in genomics.}
\label{tab:bioinformatics_case_study}
\begin{tabularx}{\textwidth}{@{} p{0.18\linewidth} p{0.26\linewidth} p{0.26\linewidth} >{\RaggedRight}X @{}}
\toprule
\textbf{Question} & \textbf{Generated Code 1 (Incorrect)} & \textbf{Generated Code 2 (Correct)} & \textbf{Analysis of Error \& Correction} \\
\midrule

% --- Column 1: Question ---
Using the 2021 CKD-EPI Creatinine equation, what is the patient's Glomerular Filtration Rate (GFR) in terms of mL/min/1.73 m²? Answer with a decimal number without unit and with a relative precision of 0.0001.

&

% --- Column 2: Incorrect Code ---
\begin{lstlisting}[language=Python]
def calculate_gfr(creatinine, age, sex):
    # Patient data from the case
    scr = float(creatinine)
    age_val = int(age)
    gfr = 175 * (scr ** -1.154) * (age_val ** -0.203)
    if sex.lower() == 'female':
        gfr = gfr * 0.742
    return gfr

\end{lstlisting}

&

% --- Column 3: Correct Code ---
\begin{lstlisting}[language=Python]
def calculate_gfr(creatinine, age, sex):
    scr = float(creatinine)
    age_val = int(age)
    k = 0.0
    alpha = 0.0
    
    # Set parameters based on sex
    if sex.lower() == 'female':
        k = 0.7
        alpha = -0.241
    elif sex.lower() == 'male':
        k = 0.9
        alpha = -0.302
    else:
        # This case is not relevant for the problem but good practice
        raise ValueError("Sex must be 'male' or 'female'")

    # Apply the 2021 CKD-EPI equation
    scr_over_k = scr / k
    min_term = (min(scr_over_k, 1.0)) ** alpha
    max_term = (max(scr_over_k, 1.0)) ** -1.200
    age_term = 0.9938 ** age_val
    gfr = 142 * min_term * max_term * age_term
    return gfr
\end{lstlisting}

&

% --- Column 4: Reason ---
Flawed Solution: Incorrectly implements the older and less accurate MDRD (Modification of Diet in Renal Disease) equation. This formula uses a single, continuous calculation.

Correct Solution: Properly implements the required 2021 CKD-EPI (Chronic Kidney Disease Epidemiology Collaboration) equation. This is a more modern and accurate formula that uses complex, conditional logic, changing the calculation based on the patient's sex and whether their serum creatinine level is above or below a specific threshold.

\\
\bottomrule
\end{tabularx}
\end{table*}

